BottleSum: Unsupervised and Self-supervised Sentence Summarization using the Information Bottleneck Principle

The principle of the Information Bottleneck (Tishby et al. 1999) is to produce a summary of information X optimized to predict some other relevant information Y. In this paper, we propose a novel approach to unsupervised sentence summarization by mapping the Information Bottleneck principle to a conditional language modelling objective: given a sentence, our approach seeks a compressed sentence that can best predict the next sentence. Our iterative algorithm under the Information Bottleneck objective searches gradually shorter subsequences of the given sentence while maximizing the probability of the next sentence conditioned on the summary. Using only pretrained language models with no direct supervision, our approach can efficiently perform extractive sentence summarization over a large corpus. Building on our unsupervised extractive summarization (BottleSumEx), we then present a new approach to self-supervised abstractive summarization (BottleSumSelf), where a transformer-based language model is trained on the output summaries of our unsupervised method. Empirical results demonstrate that our extractive method outperforms other unsupervised models on multiple automatic metrics. In addition, we find that our self-supervised abstractive model outperforms unsupervised baselines (including our own) by human evaluation along multiple attributes.

==> scratch.tex <==
%\section{Methods}
%We first describe our strategy for unsupervised sentence summary generation, then our implementation of this. Finally, we describe the model trained on our synthetic summary dataset.

%\subsection{\summfullname}
%Carrying out the optimization in eq (1) requires two parts: clear definition of a calculable summary objective $g$, and satisfaction of the information constraint over the solution set considered. For the former, we define a simple objective function inspired by the theory of Predictive Coding. The latter is ... infeasible currently ... so we instead relax the problem by considering only extractive summaries under a simple constraint to encourage adherence to this condition. 

%P1: Describe objective, justify briefly

%P2: Describe methods to satisfy constraints (extractive + filtering). Maybe mention info bottleneck (constrain-and-optimize in compression)

%P3:

%Predictive coding ... unlike much unsupervised learning, is concerned with learning representations that are predictive in some future task rather than an autoencoding objective. This motivates a very simple unsupervised objective for summarization: summary should be predictive future sentence (what details are important in context?). This offers a simple, in context definition of which details are useful, and (almost causal flavor, what do I think about S1 made S2 happen?)

%Satisfying the information constraint exactly is currently an unsolved problem (maybe cite?), and so we attempt to pose the optimization in a way that encourage it. First, \summfullname is fully abstractive, which greatly limits the number of 
%SAY HOW WE DO IT, AND JUSTIFY (maybe break into 2-3 paragraphs? Need it to be human readable to have info, need it to be informationally compressive (subset), and need details to agree) 



%MENTION: no clear way to pick params for a model on general unlablled data, so need simple objectives/constraints (could use out of domain validation like DUC but this biases us towards known domains when the value of unsupervised is being able to fit any domain)

%CONSTRAINT IDEA: parentCE makes sure no info is added, but allows for us to effectively remove words and shift their info onto other words. e.g. "I went to store" and "I went to the store" have effectively the same meaning (maybe the ambiguity of "I went to store" actually gives it more) but in the first, we effectively reconstruct "the" given the rest of it. So really, what we want is the stronger constraint that information density not increase, which actually assures SIGNIFICANT compression as you delete words 



%\subsection{Implementation}
%Keep it short, maybe 2 paragraphs. Mention: GPT-2, beam search (describe this briefly) and that we use moses tokenizer to split words. Maybe mention the window

%\section{Experiments}

==> sections/05_discussion.tex <==
\section{Discussion}

\begin{table*}[t]
    \centering
    \small
    \begin{tabular}{p{1.5cm}|p{2.9cm}p{4cm}p{5.9cm}}
    \toprule
    \textbf{Model Name} & \textbf{Model architecture} & \textbf{Target-domain data required} & \textbf{When to use} \\
    \midrule
    ABS \cite{rush2015namas} & Seq2Seq & \{(input text, output summary)\} in a very large quantity \newline for direct supervision & Large amount of in-domain data available for direct supervision. \\ 
    \midrule
    $\text{SEQ}^3$ \cite{SEQ3} & Seq2Seq2Seq
    %for summarizing and reconstruction; Language Model 
    & No supervision data needed & When there's no in-domain data available for direct-supervision, and the next sentences are \emph{not} available for sentences to be summarized. \\
    \midrule
    \bottleEx{} & Pre-trained LMs & No supervision data needed, \newline but decoding algorithm requires that the next sentence of the input sentence is available 
    & When there's no in-domain data available for direct-supervision, and the next sentences \emph{are} available for sentences to be summarized. \newline (Better than $\text{SEQ}^3$ or out-of-domain ABS.) \\
    \midrule
    \bottleSelf{} & Pre-trained LMs \newline
    (fined-tuned on data \newline induced from \bottleEx{})
    %for \bottleEx{} ; LM fine-tuned as Seq2Seq 
    & Same as above during training.  \newline  The next sentence is no longer required for testing. & Same as above, plus, a sufficient amount of raw text available in the target domain to support \bottleEx{} training. \newline (Better than \bottleEx{}). \\
    \bottomrule
    \end{tabular}
    \caption{Comparison of sentence summarization methods.} 
    %\yejin{Can we discuss pros and cons so that it's more insightful/informative? e.g., BottleEx can work with zero in-domain text, where as BottleSelf requires minimally lots of in-domain text over which BottleEx can run in advance, and Rush model is great when there's A TON OF training data but otherwise out of luck, but the sublties of bottleex is the access to the next sentence during decoding. I think we can lose the last column about pre-trained model though}
    \label{tab:comparison}
\end{table*}

Table \ref{tab:comparison} compares the training and decoding setups of the different models. 
